JESTR: Joint Embedding Space Technique for Ranking Candidate Molecules for the Annotation of Untargeted Metabolomics Data

Motivation: A major challenge in metabolomics is annotation: assigning molecular structures to mass spectral fragmentation patterns. Despite recent advances in molecule-to-spectra and in spectra-to-molecular fingerprint prediction (FP), annotation rates remain low. Results: We introduce in this paper a novel paradigm (JESTR) for annotation. Unlike prior approaches that explicitly construct molecular fingerprints or spectra, JESTR leverages the insight that molecules and their corresponding spectra are views of the same data and effectively embeds their representations in a joint space. Candidate structures are ranked based on cosine similarity between the embeddings of query spectrum and each candidate. We evaluate JESTR against mol-to-spec and spec-to-FP annotation tools on three datasets. On average, for rank@[1-5], JESTR outperforms other tools by 23.6%-71.6%. We further demonstrate the strong value of regularization with candidate molecules during training, boosting rank@1 performance by 11.4% and enhancing the model's ability to discern between target and candidate molecules. When comparing JESTR's performance against that of publicly available pretrained models of SIRIUS and CFM-ID on appropriate subsets of MassSpecGym benchmark dataset, JESTR outperforms these tools by 31% and 238%, respectively. Through JESTR, we offer a novel promising avenue towards accurate annotation, therefore unlocking valuable insights into the metabolome.

==> b_related.tex <==
%\section{Related Works}\label{related}
%\subsection{Metabolomics Data Processing and Analysis}
Metabolomics workflows are complex and require multiple prepossessing steps on the raw data files collected from the mass  spectrometry instruments. For example, MZmine \citep{schmid2023integrative} offers a wealth of tools for raw data smoothing and filtering, peak detection, alignment of various measured features, and many others to generate the spectrum data. There are now tools for \textit{de novo} molecular formula determination of a query spectrum \citep{xing2023buddy} that narrows the molecular formula search space compared to prior approaches \citep{duhrkop2019sirius}, yielding 93.0\% accuracy  for m/z values less than 400 Da, and 63.8\% accuracy for m/z $\geq$ 400 Da. 

%While each step of the data processing is important, the annotation problem is putatively the most difficult step. So far, all prior techniques mentioned in the prior section explicitly construct spectrum, fingerprints, or molecules to perform the annotation. 
Further, all techniques other than \textit{de novo} generation utilize candidate sets. 
The lack of standardized, freely available benchmark sets and the sharing of open source code has hindered the development and understanding of key techniques that can improve annotation performance.  Our evaluation of JESTR, MIST and ESP on the NPLIB1 dataset is intended to provide convincing evidence of the promise of implicit approaches. 
%\subsection{Joint Embedding Spaces}
%Since the seminal work on Siamese Networks \citep{chopra2005learning}, the idea of learning joint embedding spaces from multiple views of the same sample has taken hold. Recent work in contrastive learning \citep{chen2020simple, tian2020contrastive, khosla2020supervised} has extended the Siamese network approach significantly. Non-contrastive approaches are also proving to be very effective in learning of such embedding spaces \citep{grill2020bootstrap, assran2023self, bardes2023mc, he2022masked}. Broadly speaking, in all these approaches the key question is how to generate the paired views (either appearing naturally or generated via data augmentation); and how to ensure that paired views end up close together in the joint embedding space. Examples of pairs of input data are text/image \citep{schuhmann2022laion}, image/data-augmented image \citep{chen2020simple} and consecutive frames in a video \citep{sun2019learning}.  Our work herein recognizes that molecules and spectra are views of the same object and the views in a joint embedding space.

==> extra.tex <==
\section{PROPOSE TO REMOVE THIS SECTION: Running JESTR with 5-fold CV}
For the NPLIB1 dataset, we used the same training-validation-test split as MIST for apple to apple comparison. However, for the NIST2020 and MoNA datasets, we trained JESTR with 5-fold cross-validation split. We report results below with the standard deviation for these two datasets over the results reported in Table 2C in the main paper manuscript.

\begin{table}[h]
	\centering
	\caption{5-fold CV results for JESTR on NIST2020 and MoNA. Average performance numbers are reported along wth standard deviation} 
	{\begin{tabular}{@{}lccc@{}}\toprule 
			\multicolumn{4}{c}{\textbf{C. JESTR Results on NIST2020 and MoNA datasets}} \\
            \midrule
			Model & Top 1(\%) & Top 5(\%) & Top 20(\%)\\\midrule
			\midrule
            NIST2020-JESTR (no regularization) & 35.62(+/- 1.36) & 55.76(+/- 2.01) & 76.74(+/- 1.98)\\
			MoNA-JESTR (no regularization) & 19.28 (+/- 0.46) & 53.22 (+/- 0.56) & 84.56 (+/- 0.83)\\
			\hline 
		\end{tabular}\label{tab:results}}{}
\end{table}

\section{Comparing GAT vs GCN GNN architecture for NPLIB1 dataset}
We explored two alternative GNN architectures for the molecule encoder - GAT and GCN. GCN works better for rank@1 and hence was chosen as the architecture for the molecule encoder (Table (\ref{tab:GNN}))

\begin{table}[btp!]
\centering
\caption{Results for two different GNN architecture for molecule encoder for NPLIB1 dataset.}
{\begin{tabular}{@{}lccc@{}}\toprule Model &
Top 1(\%) & Top 5(\%) & Top 20(\%)\\\midrule
JESTR-GCN & \textbf{45.8} & 81.5 & \textbf{95.8}\\
JESTR-GAT & 44.6 & \textbf{81.6} & 94.9\\
\hline 
\end{tabular}\label{tab:GNN}}{}
\end{table}
